SMBH Seeds from Dissipative Dark Matter

The existence of supermassive black holes (SMBHs) with masses greater than $\sim 10^{9}M_{\odot}$ at high redshift ($z\gtrsim 7$) is difficult to accommodate in standard astrophysical scenarios. We study the possibility that (nearly) totally dissipative self-interacting dark matter (tdSIDM)--in rare, high density dark matter fluctuations in the early Universe--produces SMBH seeds through catastrophic collapse. We use a semi-analytic model, tested and calibrated by a series of N-body simulations of isolated dark matter halos, to compute the collapse criteria and timescale of tdSIDM halos, where dark matter loses nearly all of its kinetic energy in a single collision in the center-of-momentum frame. Applying this model to halo merger trees, we empirically assign SMBH seeds to halos and trace the formation and evolution history of SMBHs. We make predictions for the quasar luminosity function, the $M_{\rm BH}$-$\sigma_{\rm v}^{\ast}$ relation, and cosmic SMBH mass density at high redshift and compare them to observations. We find that a dissipative dark matter interaction cross-section of $\sigma/m \sim 0.05~\rm cm^2/g$ is sufficient to produce the SMBHs observed in the early Universe while remaining consistent with ordinary SMBHs in the late Universe.

==> referee_report_response.tex <==
%  
%   THIS IS THE REFEREE REPORT HERE  -- FEEL FREE TO EDIT IT
%   YOU CAN MAKE ANY CHANGES YOU WANT TO THE MANUSCRIPT letter.tex TOO WITHOUT WORRY
%   latexdiff IS USED TO KEEP TRACK OF CHANGES
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%      
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%      
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%
%
%   TO GENERATE FINAL REFEREE RESPONSE, DOWNLOAD THE PROJECT AND DO
%   latexdiff letterPreRefVersion2019-07-10.tex letter.tex > refResponse.tex
%   and then compile refResponse.tex with LaTeX
%
%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%      
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%      
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%      

{
\centering
\textbf{Referee Report Response}\\
}

{
\centering
\noindent ---------------------------------------------------------------------\\
Reviewer's Comments:\\
\noindent ---------------------------------------------------------------------\\
}
\bigskip

{\bf\textcolor{blue}{
Thanks for your thorough report. Please find below the response to the referee’s remarks
}}
\bigskip

{\it 
The manuscript "SMBH Seeds from Dissipative Dark Matter" develops, cal- ibrates using N-body simulations, and presents the results of a semi-analytic model for supermassive black hole (SMBH) seeding and growth in a dissi- pative self-interacting dark matter (dSIDM) cosmology. The paper demon- strates that dSIDM can potentially alleviate the puzzle of early and rapid SMBH growth, and it is timely given recent observational and theoretical progress on the SMBH growth and SIDM fronts. Thus, I highly recommend the manuscript for publication.
}

{\it 
{\bf [1.]} 
In the first paragraphs of the Introduction and in general through- out the paper, the Eddington limit is mostly discussed as a “hard” limit on SMBH accretion rates. Either in the Introduction or later in the text, it would be helpful to expand on the observational situation, since at least some systems are thought to accrete at super-Eddington rates (e.g., see https://arxiv.org/abs/1903.06844 and references therein).
}

\bigskip
{\bf\textcolor{blue}{
We added the discussion that super-Eddington accretion is another option for explaining the existence of those SMBHs.
}}
\bigskip

{\it 
{\bf [2.]}
In the third Introduction paragraph on elastic SIDM, it would be help- ful to discuss the characteristic relative velocity scale for dark matter particle interactions that influences the formation of the SMBHs of interest. This is necessary to fairly compare to cluster merger constraints, which are derived at relative velocites vrel 1000-2000 km/s, and would also help foreshadow the rest of the paper. As currently written, this paragraph of the Introduc- tion raises the following questions: 1. Can velocity *dependent* elastic SIDM models effectively seed SMBHs while avoiding the observational constraints in question? 2. Conversely, do non-dissipative SIDM models informed by low-redshift observations (including cluster mergers, cluster shapes, dwarf galaxy profiles, etc.) impact SMBH seeding?
}

\bigskip
{\bf\textcolor{blue}{
The virial velocities of the rare halos we studied are in range 200-2000 km/s, which overlaps a bit with the relative velocities of the bullet clusters. A velocity dependent cross-section might avoid those constraints but we did not study it quantitatively. We have added the discussion in the introduction. Non-dissipative SIDM, if consistent with low-redshift observations, should have little impact on the SMBH seeding because the collapse timescale is too long. There are several ways to accelerate it and velocity-dependent cross-section is a possibility.}}
\bigskip

{\it 
{\bf [3.]} 
The assumption that fdiss = 1 is reasonable given the scope of this paper, but a discussion of its implications (perhaps in a Discussion section preceding the Conclusions) would be informative. For example, what level of degeneracy is expected between cross section and fdiss for models that efficiently seed SMBHs?
}
\bigskip

{\bf\textcolor{blue}{
The degeneracy of $f_{\rm diss}$ with the cross section is now discussed at the end of section 4. The only relevant parameter in this model is $f_{\rm diss}\epsilon \sigma/m$ since this is the only parameter related to the physical model that appears in the equation that gives the dissipation timescale.
}}
\bigskip

{\it 
{\bf [4.]}
I recommend specifying (perhaps in a Table) relevant information on the simulations used to calibrate the semi-analytic model (e.g., number of simulations, halo mass range, simulation parameters like particle mass and softening scale, etc.). I also recommend more clearly describing the envi- ronment of the simulated halos (e.g., are they completely isolated, what assumptions are made about their dark matter accretion rates, and so on?).
}

\bigskip
{\bf\textcolor{blue}{
Thanks for the suggestion! Now a summary of the numerical parameters in the N-body simulation is added at the beginning of Section 2.
}}
\bigskip

{\it 
{\bf [5.]}
The universal collapsed mass fraction is an interesting finding. Given its emphasis throughout the paper, additional discussion on the following aspects may be helpful: 1. For larger cross sections or longer integration times, is fcoll expected to remain nearly constant for lower-mass halos (and even for extremely small halos), if baryons are neglected? 2. How significant are the expected deviations from self-similarity due to baryonic physics, especially given that the initial SMBH seeds probe ex- tremely small physical scales on which baryons may be prevalent? This is discussed briefly in the context of c(M) near Eq. 3.1, but also potentially impacts fcoll. 3. Would fcoll remain universal for fdiss < 1, and how is it expected to depend on fdiss? Would it remain universal for velocity-dependent dSIDM momentum transfer?
}

\bigskip
{\bf\textcolor{blue}{
Thanks for pointing this out. These are very interesting questions. Here are our responses. 1. We have tested different cross-sections in Appendix C and they have nearly the same collapse fraction. Therefore we conclude that cross-section will not break the universality. 2. We have not studied the baryonic effect quantitatively so we do not know if the collapse fraction will be changed by it. In the context of c(M), baryonic physics can be relevant in the merger tree model that determines the scatter on the concentrations. 3. This is indeed a very important point. We have not tested this numerically but it should not change this collapse fraction based on our arguments in Appendix C, which only rely on gravitational instabilities and the NFW profile. We have added these discussions in Appendix C.
}}
\bigskip

{\it 
{\bf [6.]}
— Figure 3 would benefit from clearer labels (e.g., a legend stating what the points with errorbars and dashed lines respectively represent). Also, the discrepancies near $10^{13}\,{\rm M}_{\odot}$ at z = 6 seem statistically significant and are surprising given the good agreement at lower and higher z. Is there a qualitative explanation of this?
}

\bigskip
{\bf\textcolor{blue}{
We add labels to Figure 3 to clarify points with error bars and lines. We also add descriptions to the caption. The discrepancy near $10^{13}\,{\rm M}_{\odot}$ is mainly due to stochastic effects of merger trees. In the figure, the error bar only represents poisson errors from limited number of trees sampled in a given mass range. However, when tracing back the merger trees to higher redshift, the stochastic effects in merger histories become important and introduce additional errors. This would particularly happen at the massive end. For example, if we sample a median mass growth history of a final halo at $z=4$ and we miss halos with rapid/slow growth histories. Missing halos with rapid growth histories will not matter since they give lower mass halos at high redshift and become subdominant compared to contributions from lower mass trees. However, missing halos with slow growth histories will matter since it should give more massive halos at high redshift. Missing this part could lead to dips in the halo mass function. We have tested this by doubling the number of trees sampled at $z=4$ and the discrepancy is alleviated. 
}}
\bigskip

{\it 
{\bf [7.]}
It may be helpful to discuss the most relevant caveats associated with treating the evolution of merging BH binaries as a single BH immediately after the halo merger.
}

\bigskip
{\bf\textcolor{blue}{
We enrich the discussion about this at the end of the first paragraph in Section 3.1.
}}
\bigskip

{\it 
{\bf [8.]}
Figure 4: If possible, I would find a third line with the $\sigma/m = 0$ prediction helpful (same comment for Figure 5). Given the range of uncertainties that go into translating SMBH abundance to the quasar luminosity function as discussed in the text, a brief description of the assumptions used to derive the shaded regions in this figure would be helpful.
}

\bigskip
{\bf\textcolor{blue}{
We are not sure about the first part of the comment, since the $\sigma/m = 0$ will not give SMBH seeds in this model. Regarding the second part of the comment, we add a footnote discussing how the shaded regions were derived.
}}
\bigskip

{\it 
{\bf [9.]}
On page 20, I recommend editing the mention of LSST following this naming guide: https://project.lsst.org/documents/name-use-guide.
}

\bigskip
{\bf\textcolor{blue}{
The name has been corrected to "the Rubin Observatory Legacy Survey of Space and Time (LSST)".
}}
\bigskip

{\it 
{\bf [10.]}
Figure 7: Although the $\sigma/m = 0.05$ model performs better than the $\sigma/m = 1$ model in this parameter space, it still seems to underpredict the scatter in the observed M-$\sigma$ relation. In the text or figure caption, a discussion of which approximations in this paper are expected to increase the predicted scatter when modeled more carefully may be helpful.
}

\bigskip
{\bf\textcolor{blue}{
The scatter is underpredicted mainly due to the fixed relation we use to link $V_{\rm c}$ to $\sigma^{\ast}_{\rm v}$. We add a discussion about the scatter and estimate a proper value of scatter based on low redshift observations. 
}}
\bigskip

{\it 
{\bf [11.]}
The end of Section 4 states that “The discussion here demonstrates that there exists a parameter space of dissipative dark matter where the predictions are consistent with observations at both high and low redshift.” Given the sizable number of astrophysical parameters that were held fixed at fiducial values in this analysis, it would be helpful to reiterate the most important astrophysical degeneracies here and to discuss whether there are observational paths that will help break them.
}

\bigskip
{\bf\textcolor{blue}{
We add this discussion at the end of Section 3.2.
}}
\bigskip

{\it 
{\bf [12.]}
In the Conclusions or in a preceding Discussion section, I recommend discussing the implications that dSIDM models like those studied here have for cosmological observables beyond the SMBH seeding/growth paradigm, in order to place them in a broader observational and phenomenological con- text. For example, the Shen et al. (2021) hydrodynamic dSIDM simulations demonstrate that halo density profiles, kinematics, and shapes can notice- ably differ from CDM, even for smaller values of sigma/m and fdiss than considered in this paper. Thus, the models considered here may significantly affect structure formation and galactic dynamics relative to CDM. Although other recent SIDM work mostly focuses on non-dissipative self-interactions, effects explored in the literature including accelerated core collapse and enhanced subhalo disruption are likely to be present (and perhaps exacerbated) in dSIDM. In turn, a discussion of potential observational signatures of such effects (e.g., in strong gravitational lensing and dwarf galaxies) is warranted. Such a discussion would help guide the way for future work to test and compare the predictions of dSIDM and SIDM, and CDM using a variety of observational techniques.
}

\bigskip
{\bf\textcolor{blue}{
We add the Section 5 to discuss existing constraints on dSIDM from dwarf galaxies and explain that our model is still consistent with these studies. We highlight the potential that dSIDM can created observational signatures in strong gravitational lensing.
}}
\bigskip

\setcounter{figure}{0}
\clearpage
\newpage
